Interactive Language: Talking to Robots in Real Time

We present a framework for building interactive, real-time, natural language-instructable robots in the real world, and we open source related assets (dataset, environment, benchmark, and policies). Trained with behavioral cloning on a dataset of hundreds of thousands of language-annotated trajectories, a produced policy can proficiently execute an order of magnitude more commands than previous works: specifically we estimate a 93.5% success rate on a set of 87,000 unique natural language strings specifying raw end-to-end visuo-linguo-motor skills in the real world. We find that the same policy is capable of being guided by a human via real-time language to address a wide range of precise long-horizon rearrangement goals, e.g. "make a smiley face out of blocks". The dataset we release comprises nearly 600,000 language-labeled trajectories, an order of magnitude larger than prior available datasets. We hope the demonstrated results and associated assets enable further advancement of helpful, capable, natural-language-interactable robots. See videos at https://interactive-language.github.io.

==> long_horizon_v0.tex <==
\textbf{Long horizon goal reaching}.
Next we aim to see whether humans can guide \algname policies through a wide range of multi-step compositional rearrangements.
We define over 100,000 language-distinct compositional goal states on our tabletop from 11 high level families (e.g. make high-level shapes, sort by color, place all blocks in specific locations, arrange into lines, etc.), then sample 20 uniformly from all 11. See Figure~\ref{fig:new_capabilities} for examples of different goal states. We evaluate each long horizon goal 3 times from randomly reset board states, yielding 60 total evaluations of a single policy.
We report success rates in Table~\ref{tab:long-horizon}.
We see that our policy obtains an $85.0\%$ expected average success rate on this diverse set of goals, $95\% \; CI \; [69.35\%, 100.00\%]$. 
% V0:
We note that for a policy with a \textit{single-task} average success of $93.5\%$, the expected \textit{cumulative} success over 15 \textit{random} sequential instructions should drop to $\sim36\%$ (if the policy performs no sub-task re-planning or does not receive feedback throughout the episode), yet policies under \algname guidance achieve $\sim85\%$ expected success.
This is important as it shows that even when a low-level policy is imperfect, occasional situation-specific corrections made possible by real-time language allow a robot to achieve better than anticipated long horizon outcomes. These results are best appreciated by watching the videos here: \todo{link to videos}. 

\textbf{Open-loop vs real-time language feedback}. Here we attempt to quantify the importance of being able to provide \textit{real-time} feedback, over the more common ``open-loop" evaluation setting where the sequence of subgoals is decided up front \cite{gupta2019relay, stepputtis2020language,lynch2020language, ahn2022can}.
We hypothesize that many of the tasks in our environment might require several rounds of iterative and interactive specification, due to the stochastic nature of single-point-of-contact pushing.
We perform the same evaluation as in the previous section, but the human operator commits up front to the set and order of commands they will provide.
We presented results for this ablation in Table~\ref{tab:long-horizon}, finding that performance deteriorates from 85\% to 25\% when real-time language is removed. This shows that for %stochastic,
contact-rich tasks like the ones studied in this work, success depends on sufficient \textit{real-time feedback}---not only for the low-level policy, but also for and the agent providing it instructions.

==> prf_intro.tex <==
The goal of building a robot that can follow a diverse array of natural language instructions has been a longstanding goal of AI research, since at least the SHRDLU experiments starting in the late 1960s.
While recent research on this topic has been abundant,
few efforts have actually produced a robot that (i) exists in the real world, and (ii) can capably respond to a large number of rich, diverse natural language commands -- for which we expect this number to continue to grow as the research frontier progresses. %While chaining together a finite set of skills in diverse ways can expand the set of natural language, it's not apparent this can addresss fine-grained sensorimotor skills such as {\em{``gently nudge thing A in between things B and C''}}. This number
%For the number of addressable skills, one may expect that the research frontier will continue to grow this number, whether through sequencing skills, or growing the number of raw visuo-linguo-motor skills themselves.
We are also particularly interested in (iii), the ability to {\em{interactively}} \cite{bohg2017interactive} respond to natural language commands, by which we mean that the robot fluidly responds in-the-moment to new natural language instructions during task execution, including during contact-rich manipulation tasks.  Although we should expect such a robot to be possible given current methods, typically natural-language-interactable robots are often slow and instead utilize simplifying self-resetting behaviors, or blocking parameterized skills, that prohibit this type of real-time, live interaction.

\begin{figure}[t]
    \noindent
    \centering
    \includegraphics[width=\linewidth]{figs/money_shot/moneyshot-2.pdf}
    \caption{\textbf{Guiding a physical robot iteratively and interactively with natural language.} Over the course of 5 minutes, a human guides a robot to precisely rearrange objects a table into a desired shape, with real-time natural language as the only control mechanism. Language is used to specify new subgoals on-the-fly, offer real-time corrections, or to constrain the motions of the agent towards safer behavior (e.g. ``slide the triangle \textit{slowly} left").}
    \label{fig:moneyshot}
\end{figure}

In this paper we demonstrate a real-world, real-time-interactable, natural-language-instructable robot that by certain metrics of scale is at an order of magnitude larger than prior works, and to accelerate further research we accordingly provide our associated recipe, dataset, hardware enironment description, simulated analogue environment, and benchmark.  In terms of scale, the robot exhibits raw end-to-end sensorimotor skills that can address 87,000 unique strings at an estimated 93\% success rate, with real-time continuous control, and is capable of chaining raw skills to hundreds of thousands of language-distinct states in its environment.  This robot exists in an environment (Fig. 1) which we have designed to present a tractable yet difficult level of challenge (feedback-rich control, many objects, subtle natural language instructions) while enabling safe, fast control in the real world. The learning algorithm recipe itself is intentionally simple, and instead the complexity of this effort was primarily in the data effort itself, for which we detail insights and techniques. We hope the dataset and benchmark may catalyze further work which may improve on our demonstrated sample complexity and performance.

Beyond just demonstrating capabilities and providing associated assets, we also utilize these capabilities to study nonobvious benefits of such a proficient robot.  For one, we show that through occasional human natural-language feedback, the robot can accomplish long-horizon, complex rearrangements such as {\em{``put the blocks into a smiley face with green eyes''}} that require multiple minutes of precise coordinated control. The competency of the robot policy also enables simultaneous, live multi-robot instruction -- in which a single human can guide multiple real-time robots.

%a robot that meets the following criteria has remained elusive: 
%(i) exist in the real world,(ii) , and (iii) fluidly respond in-the-moment to natural language commands interactively during task execution.  This short list of criteria imposes considerable challenges: as just one example, (iii) implies that blocking move-until-done motion primitives, or self-resetting behaviors which interrupt task execution, may not be permissible.




==> v0_intro.tex <==
% A long term goal is generalist robots operating in human spaces.
An ambitious long-term goal in robot learning is the concept of robot \textit{generalists} — robots that inhabit human spaces and are capable of being instructed to carry out a wide range of autonomous behaviors. 
% 2 focuses: multitask visual control, natural language conditioning.
Two lines of work that have made significant progress toward this goal are imitation learning \cite{pomerleau1989alvinn, billard2008robot} of multi-task visuomotor control \cite{levine2016end,rahmatizadeh2018vision,zhang2018deep}, which allows robots to learn numerous skills directly from general onboard sensors, and natural language conditioning \cite{branavan2009reinforcement, tellex2011understanding, chen2011learning, matuszek2013learning,hill2019emergent,lynch2020language}, which allows non-expert end users to specify these behaviors in a familiar format.

% The way we use language with robots is currently non-interactive.
However, there are still significant differences between how humans instruct robots, and how we instruct each other.
Robots today often receive instructions from a human operator asynchronously \cite{stepputtis2020language, jang2022bc}, and without additional instructional feedback.
This form of action specification can be constraining, especially in dynamic human environments, as it provides limited support for unexpected events.
Humans directing other humans, on the other hand, handle complex and changing conditions with ease by specifying our aims \textit{interactively}. We quickly define new subtasks on-the-fly based on recent observations, offer real-time corrections, and put constraints on each other's behavior when the situation calls for it (e.g.  “move  your  arm  down \textit{slowly}”).

% This type of natural feedback could be beneficial to robots, particularly \textit{learning} robots that do not always do what we desire. 
% Existing modes of correction are inflexible. Natural language correction unlocks: 1) non-experts customizing robot behavior, 2) free new source of competency for learning robots.
% Historical modes of robot correction involve trained operators \todo{cite}, providing corrections via joysticks \todo{cite} or full-robot teleoperation \todo{cite}.
% A guiding principle in many studies of robot learning is that humans should not need to be a programmer, or rely on a programmer, to request actions from a robot or alter robot behavior.
% Historical modes of robot correction involve trained operators \todo{cite}, providing corrections via joysticks \todo{cite} or full-robot teleoperation \todo{cite}.

There are at least two advantages to choosing natural language as the format for interactive robot control, as opposed to prior methods like joystick control \cite{spencer2020learning}, kinesthetic teaching \cite{kormushev2011imitation} or full-robot teleoperation \cite{rakita2018autonomous}.
First, language allows humans with no robot training to quickly customize robot behavior mid-execution, or guide robots through complex multi-stage tasks.
Second, language allows learning robots to leverage a large new source of competence to get out of local optima or avoid unsafe behavior. For a robot equipped with an interactive language interface, any user in a robot's environment, even non-technical ones, becomes a potential teacher.
% In future deployed scenarios, non-experts must be able to customize online robot behavior quickly and through familiar means. Natural language potentially unlocks a new category of robot teachers---people not trained in teleoperation who can nevertheless guide an autonomous robot through a complicated multi-stage tasks.
% The promise of employing natural language as the format for live robot corrections, in comparison to earlier forms of test-time feedback like joystick control \todo{cite} or teleoperation \todo{cite}, is to dramatically scale the amount of corrective feedback available to the robot. Any user in a robot's environment, including non-technical ones,  becomes a possible new source of test-time competency.
% Interactive language can be used to specify compositional target behaviors(e.g. “place the red circle on the left side of the green one”),to offer online  corrections (e.g.  “move  your  arm  down  a little”), or to specify behavioral constraints(e.g. “move the cube  down slowly”).
% The historical importance of feedback.
% Feedback is a fundamentally important concept more broadly in robot learning.
% A key insight from control \todo{cite} is that a policy needs to receive sufficient \textit{feedback} during execution to succeed, particularly for stochastic tasks.
% A natural step forward for instruction following robots is to start benefiting from real-time feedback in their language conditioning, in the same way that closed-loop policies have benefited from real-time feedback in their observations.

% \begin{figure}[h!]
%     \noindent
%     \centering
%     \includegraphics[width=\linewidth]{scale=0.5,width=\textwidth]{figs/money_shot/moneyshot-2.pdf}
%     \caption{\textbf{Interactive natural language conditioned control of a physical robot.} Over the course of 5 minutes, a human guides a high-rate visuomotor robot to precisely rearrange objects a table, with real-time natural language as the only control mechanism. Language is used to specify new subgoals on-the-fly, offer real-time corrections of unsafe or undesirable behavior, or constrain the motions of the agent (e.g. ``slide the triangle \textit{slowly} left").}
%     \label{fig:moneyshot}
% \end{figure}

\begin{figure}[t]
    \noindent
    \centering
    \includegraphics[width=\linewidth]{figs/money_shot/moneyshot-2.pdf}
    \caption{\textbf{Guiding a physical robot iteratively and interactively with natural language.} Over the course of 5 minutes, a human guides a robot to precisely rearrange objects a table into a desired shape, with real-time natural language as the only control mechanism. Language is used to specify new subgoals on-the-fly, offer real-time corrections, or to constrain the motions of the agent towards safer behavior (e.g. ``slide the triangle \textit{slowly} left").}
    \label{fig:moneyshot}
\end{figure}

% Introduce our setting clearly.
In this work, we investigate learning an \textit{interactive natural language interface for high-rate manipulation} (Figure~\ref{fig:moneyshot}). 
We cast this as an large scale imitation learning \cite{Pomerleau_behavior_cloning,osa2018algorithmic} problem, implemented on robots tasked with rearranging objects on physical tabletops.  While we restrict our attention to a discrete set of objects, we find this setting nevertheless incorporates multiple difficult subproblems in robot learning: (1) High-rate visuomotor control from RGB pixels. 
% We perform asynchronous inference and control at 5Hz, requiring $\sim$1500 sequential robot decisions in a typical evaluation episode. 
(2) Open vocabulary language conditioning. We study 87k unique language-conditionable skills learned by a single robot (Figure~\ref{fig:short_horizon_behaviors}).
(3) Contact-rich, real world tasks with stochastic dynamics (i.e. single-point-of-contact block pushing). (4) Long-horizon, large cardinality goal reaching. We study whether a single policy can be guided over a long horizon with language to address over $\sim$100,000 multi-stage rearrangement goals. e.g. ``make a smiley face", ``group all the blocks by color" (Figure~\ref{fig:long_horizon_goals}).
% In this 8-block environment, due to their shapes, colors, and configurations, we identify at least 100,000 possible variations of language distinguishable goal states, e.g. ``make a smiley face", ``group all the blocks by color" \todo{point to where this is defined}.
(5) Ambiguous language grounding. The instructions we study (e.g. ``nudge the cube a bit closer to the right side of the hexagon") require agents to ground \cite{winograd1972understanding} discrete object properties, precise spatial relationships, and ambiguous constraints like ``nudge" or ``a bit closer" in their high-dimensional observations and action sequences. Multiple instructions can describe a single behavior (e.g. “push the triangle to the cube” and “make the triangle and cube touch”), and a single instruction can describe multiple valid behaviors (e.g. ``group up the blue blocks").
% This grounded language comprehension is a notoriously difficult problem across broader machine learning \todo{cite}.

